ZIP-FIT: Embedding-Free Data Selection via Compression-Based Alignment

Data selection is crucial for optimizing language model (LM) performance on specific tasks, yet most existing methods fail to effectively consider the target task distribution. Current approaches either ignore task-specific requirements entirely or rely on approximations that fail to capture the nuanced patterns needed for tasks like Autoformalization or code generation. Methods that do consider the target distribution often rely on simplistic, sometimes noisy, representations, like hashed n-gram features, which can lead to collisions and introduce noise. We introduce ZIP-FIT, a data selection framework that uses gzip compression to directly measure alignment between potential training data and the target task distribution. In extensive evaluations on Autoformalization and Python code generation, ZIP-FIT significantly outperforms leading baselines like DSIR and D4. Models trained on ZIP-FIT-selected data achieve their lowest cross-entropy loss up to 85.1\% faster than baselines, demonstrating that better task alignment leads to more efficient learning. In addition, ZIP-FIT performs selection up to 65.8\% faster than DSIR and two orders of magnitude faster than D4. Notably, ZIP-FIT shows that smaller, well-aligned datasets often outperform larger but less targeted ones, demonstrating that a small amount of higher quality data is superior to a large amount of lower quality data. Our results imply that task-aware data selection is crucial for efficient domain adaptation, and that compression offers a principled way to measure task alignment. By showing that targeted data selection can dramatically improve task-specific performance, our work provides new insights into the relationship between data quality, task alignment, and model learning efficiency.

==> 00_main.tex <==
 % \documentclass{article} % For LaTeX2e
\usepackage{iclr2025_conference,times}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\input{math_commands.tex}

\usepackage{hyperref}
\usepackage{url}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{xcolor}
\usepackage{mdframed}

\newcommand{\rylan}[1]{\textcolor{purple}{RS: #1}}

\title{ZIP-FIT: Embedding-Free Data Selection via Compression-Based Alignment}

% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

% https://chatgpt.com/c/671709cb-c7d4-8001-bbd5-48781d995543
\author{%
  \textbf{Elyas Obbad}\textsuperscript{1}, \textbf{Iddah Mlauzi}\textsuperscript{1}, \textbf{Brando Miranda}\textsuperscript{1}, \\
  \textbf{Kamal Obbad}\textsuperscript{3}, \textbf{Rylan Schaeffer}\textsuperscript{1}, \textbf{Suhana Bedi}\textsuperscript{2}, \textbf{Sanmi Koyejo}\textsuperscript{1} \\
  \texttt{\{eobbad, iddah, brando9, sanmi\}@cs.stanford.edu} \\
  \textsuperscript{1}Department of Computer Science, Stanford University\\
  \textsuperscript{2}Department of Biomedical Data Science, Stanford School of Medicine\\
  \textsuperscript{3}Stanford Biophysics Program, Stanford School of Medicine\\
  % \texttt{\{kobbad, suhana\}@stanford.edu}
}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

% \iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
\begin{document}

\maketitle

\input{01_abstract}
\input{02_introduction}
\input{03_zip_fit}
\input{04_interventional}
\input{05_efficient}
\input{06_misalignment}
\input{07_conclusion} 

\clearpage

\bibliography{iclr2025_conference,references_rylan}
\bibliographystyle{iclr2025_conference}

\clearpage

\appendix

\input{99_appendix}


\end{document}

